On Network Embedding for Machine Learning on Road Networks: A Case Study on the Danish Road Network

Road networks are a type of spatial network, where edges may be associated with qualitative information such as road type and speed limit. Unfortunately, such information is often incomplete; for instance, OpenStreetMap only has speed limits for 13% of all Danish road segments. This is problematic for analysis tasks that rely on such information for machine learning. To enable machine learning in such circumstances, one may consider the application of network embedding methods to extract structural information from the network. However, these methods have so far mostly been used in the context of social networks, which differ significantly from road networks in terms of, e.g., node degree and level of homophily (which are key to the performance of many network embedding methods). We analyze the use of network embedding methods, specifically node2vec, for learning road segment embeddings in road networks. Due to the often limited availability of information on other relevant road characteristics, the analysis focuses on leveraging the spatial network structure. Our results suggest that network embedding methods can indeed be used for deriving relevant network features (that may, e.g, be used for predicting speed limits), but that the qualities of the embeddings differ from embeddings for social networks.

==> illustrations/road-network-intersections.tex <==
\begin{figure}    
    \centering
\begin{subfigure}{\columnwidth}
  \centering
  \begin{tikzpicture}
    \matrix [draw] at (current bounding box.south) {
      \node [fill={rgb:red,255}, label=right:Secondary] {}; &
      \node [fill={rgb:blue,255}, label=right:Tertiary] {}; &
      \node [fill={rgb:blue, 139; green, 139}, label=right:Residential] {}; \\
  };
  \end{tikzpicture}
  \vspace{0.15cm}
\end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \begin{tikzpicture}
      \def \radius {0.8 cm}
      \def \width {0.4 cm}
      \def \edgewidth {2pt}
      \def \edgelabeloffset {0.01cm}
      
      \node[draw, circle, text width=1.5cm, align=center] (roadnetwork) at (0, 0) {Large \\ Road \\ Network};
      
      % Left Intersection
      \node[draw, circle, left = \radius of roadnetwork, text width = \width] (intersection1) {};
      \node[draw, circle, left = \radius of intersection1, text width = \width] (west1) {};
      \node[draw, circle, above = \radius of intersection1, text width = \width] (north1) {};
      \node[draw, circle, below = \radius of intersection1, text width = \width] (south1) {};
      
      \draw[line width=\edgewidth, color={rgb:blue, 139;green, 139}, text=black] (roadnetwork) -- (intersection1) node [midway, fill=white, below=\edgelabeloffset] {$s_3$};
      \draw[line width=\edgewidth, color={rgb:blue, 255}, text=black] (intersection1) -- (west1) node [midway, fill=white, above=\edgelabeloffset] {$s_1$};
      \draw[line width=\edgewidth, color={rgb:red, 255}, text=black] (intersection1) -- (north1) node [midway, fill=white, right=\edgelabeloffset] {$s_2$};
      \draw[line width=\edgewidth, color={rgb:red, 255}, text=black] (intersection1) -- (south1) node [midway, fill=white, left=\edgelabeloffset] {$s_4$};
     
      % Right Intersection
      \node[draw, circle, right = \radius of roadnetwork, text width = \width] (intersection2) {};
      \node[draw, circle, above = \radius of intersection2, text width = \width] (north2) {};
      \node[draw, circle, below = \radius of intersection2, text width = \width] (south2) {};
      \node[draw, circle, right = \radius of intersection2, text width = \width] (east2) {};
      
      \draw[line width=\edgewidth, color={rgb:blue, 255}, text=black] (roadnetwork) -- (intersection2) node [midway, fill=white, above=\edgelabeloffset] {$s_5$};
      \draw[line width=\edgewidth, color={rgb:blue, 255}, text=black] (intersection2) -- (east2) node [midway, fill=white, below=\edgelabeloffset] {$s_7$};
      \draw[line width=\edgewidth, color={rgb:red, 255}, text=black] (intersection2) -- (north2) node [midway, fill=white, right=\edgelabeloffset] {$s_6$};
      \draw[line width=\edgewidth, color={rgb:red, 255}, text=black] (intersection2) -- (south2) node [midway, fill=white, left=\edgelabeloffset] {$s_8$};
    \end{tikzpicture}
  \end{subfigure}
  \caption{Two similar 4-way intersections far apart in a road network. Road segments are color-coded according to their \gls{osm} category.\label{fig:road-network-intersections}}
\end{figure}


==> road_network_embedding.tex <==
\section{Selected Road Network Embedding Methods}
In principle, any road network analytics task that rely on machine learning could stand to benefit from \gls{rne}. In this section we review some road network analytics tasks found in the recent scientific literature and classify them as either local or non-local as described in \cref{sec:network-embedding}.

As an example of a non-local task, \citet{trajectory-regression} present a machine learning approach to predict time-variant travel speeds on road segments. Predicting travel speeds is a non-local task since it is often the case that travel speeds are similar in different areas of the road network. For instance, two motorway segments in different parts of a country are likely to exhibit similar travel speeds during the day. Conversely, a motorway exit segment are adjacent to a motorway and a highway or city segment which all tend to have different speed limits and thus different travel speeds.

As an example of a local task, \citet{road2vec} use embeddings to select road segments as a preprocessing step for a traffic forecasting model. Given a road segment, the task is to select nearby road segments that have similar traffic conditions. The selected road segments are subsequently used for a traffic forecasting task where the travel speed on a road segment during a future time interval is predicted based on the current travel speed of the road segment itself and similar road segments.
We now review applications for \gls{rne}. Current applications either assume the existence of an embedding method, whether through feature engineering or feature learning, or build an embedding method for the specific task. Although such task-specific embedding methods may be more generally applicable, they have not been designed nor demonstrated to do so. We therefore do not categorize them as \gls{rne} methods.

Trajectory regression

broadly be categorized as either embedding-reliant or embedding-building.  Various embedding methods to embed road network elements have already been published, but these have been designed with specific tasks in mind and thus lack the generality to be proper \gls{rne} methods. In this meth
Some road network embedding methods do exist, but have been designed for specific tasks and thus it is hard.
Some work exists within the road
In the following we review some existing road network embedding methods and possible 
\outline{Roughly half a page describing the current state-of-the-art.}
We define \glsfirst{rne} broadly as the embedding of road network elements, such as intersections, road segments, points of interest, routes, and trajectories. There has been some applications of \gls{rne}, but they have been designed for and applied to specific tasks, making their applicability for other tasks questionable. In this section, we first review existing road network embedding methods. We then look to applications in the current research and finally we describe some prospective opportunities for road network embedding.
\csj{Readers do not know what an embedding is. How do general and task-specific embeddings differ?}

\subsection{Existing Applications}

\subsection{State-of-the-Art}
\outline{direct and indirect applications?}
\subsection{Traffic Forecasting}
Road2Vec~\citep{road2vec} learn embeddings of road segments for traffic forecasting. The approach is quite similar to the structural proximity embedding methods, except that rather than sampling walks consisting of nodes they use vehicle trajectories consisting of road segments. The intuition is that if road segments often co-occur in vehicle trajectories then they are likely strongly correlated\todo{something with correlated speeds}. This also implies that connected segments are similar, i.e., the network exhibits homophily. They achieve convincing results, but their method relies on the set of vehicle trajectories used for learning to cover all road segment in their network. This cannot be expected in general~\citep{yang2014using}.

\subsection{Querying}
\citet{Shahabi2003} use embedding of intersections to improve the accuracy of KNN queries to find the nearest points of interest for moving vehicles. Specifically, they embed intersections s.t.\ the distance the shortest-path distance between two intersections is better approximated than the Euclidean distance between their geographical points. \citet{Liu11} further extend this approach further to handle private KNN-queries where the exact location of a vehicle is hidden.
\argument{Liu11 says that it is an efficient way to compute network distance}
% \citet{lsmrn} use matrix factorization to learn node embeddings directly optimized to predict time-varying traffic.


\subsection{Potential Applications}
Trajectory regression
Path-dependent routing




 - Embedding of various road network elements
  - Road2Vec~\citep{road2vec}
      \argument{Road2Vec uses structural proximity whereas this is a problem for trajectory regression. This requires flexibility.}
  - LSM-RN: https://arxiv.org/pdf/1602.04301.pdf
  - Privacy~\citep{Liu2011}
  - Road network generation~\citep{Zhou2015} 

  \subsection{Other applications}

